Phase transition in compressible Ising systems at fixed volume

Using a Ginzburg-Landau model, we study the phase transition behavior of compressible Ising systems at constant volume by varying the temperature $T$ and the applied magnetic field $h$. We show that two phases can coexist macroscopically in equilibrium within a closed region in the $T$-$h$ plane. It occurence is favored near tricriticality. We find a field-induced critical point, where the correlation length diverges, the difference of the coexisting two phases and the surface tension vanish, but the isothermal magnetic susceptibility does not diverge in the mean field theory. We also investigate phase ordering numerically.

==> Makefile <==
OBJECT = intermediate
TODAY=`date +%m%d`

all:
	platex ${OBJECT}.tex
	platex ${OBJECT}.tex
run:all
	#open -a mxdvi ${OBJECT}.dvi
	xdvi ${OBJECT}.dvi &
ps:all
	dvips -o ${OBJECT}.ps ${OBJECT}.dvi
	gv ${OBJECT}.ps &
pdf:all
	dvipdfmx ${OBJECT}.dvi
	open -a preview ${OBJECT}.pdf
clean :
	rm -f *.o *.il *.mod *.ppm *.tga *.log *.dat gmon.out mpeg.param
erase : clean
	rm -f *~ *.bak core *.ps *.aux *.dvi *.log
	rm -f *.tgz
pack : erase
	pwd | sed -e 's/.*\///' | (cd ..; xargs -I DIR tar cvz --exclude .svn -f DIR${TODAY}.tgz DIR)
.tex.dvi :
	platex $<

